Solo: Data Discovery Using Natural Language Questions Via A Self-Supervised Approach

Most deployed data discovery systems, such as Google Datasets, and open data portals only support keyword search. Keyword search is geared towards general audiences but limits the types of queries the systems can answer. We propose a new system that lets users write natural language questions directly. A major barrier to using this learned data discovery system is it needs expensive-to-collect training data, thus limiting its utility. In this paper, we introduce a self-supervised approach to assemble training datasets and train learned discovery systems without human intervention. It requires addressing several challenges, including the design of self-supervised strategies for data discovery, table representation strategies to feed to the models, and relevance models that work well with the synthetically generated questions. We combine all the above contributions into a system, Solo, that solves the problem end to end. The evaluation results demonstrate the new techniques outperform state-of-the-art approaches on well-known benchmarks. All in all, the technique is a stepping stone towards building learned discovery systems. The code is open-sourced at https://github.com/TheDataStation/solo

==> sections/relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

\notefb{R3O5. The discussion of related work is not accurate. Based on the problem definition in Section 2.2, other studies about natural language query interface over database, such as [26], should also be included into the category of "non-learned system". Meanwhile, the works introduced in "learned systems" are actually about the topic of natural language table retrieval (NLTR), which is not data discovery and also not strictly align with the problem definition. The authors should reorganize the related work section and explain in more details about the relationship between previous works and this work.}

\notera{to integrate}

We separate data discovery solutions into two categories: \emph{non-learned} and
\emph{learned}. 

\noindent\textbf{Non-learned discovery systems}~\cite{fernandez2018aurum,
castelo2021auctus, yakout2012infogather, halevy2016goods, chapman2020dataset}
rely on indices to perform efficient search over large table collections. They
often expose an API~\cite{fernandez2018aurum} to perform sophisticated discovery
tasks such as identifying similar, unionable, and joinable
tables~\cite{fernandez2018aurum, castelo2021auctus, nargesian2018table} or a
keyword search interface~\cite{brickley2019google, halevy2016goods} to identify
matching tables. None of them offers a natural language question interface.

\noindent\textbf{Learned discovery systems} support natural language question
retrieval~\cite{sun2016table, herzig2021open, wang2021retrieving} but do not
offer the more sophisticated functionality of \emph{non-learned} systems. They
consist of two stages: \emph{first-stage retrieval} and \emph{second-stage
ranking}~\cite{sun2016table}.  The first-stage retrieval is implemented by an
index designed to identify a narrow set of relevant tables in a scalable way.
The index can be sparse, such as those based on
\textsf{BM25}~\cite{robertson2009probabilistic} or dense, that model tables as
distributed representations (vectors). For example,
\textsf{OpenDTR}~\cite{herzig2021open} uses dense indexes. It learns a vector
representation for each table and for the question using a large training corpus
of <$q,T_i^*$> pairs. Then, offline, it uses a \emph{Table Encoder} component
to obtain and index the vector representation of the tables. Online, it uses a
\emph{Question Encoder} to obtain the vector representation of the question and
then it finds the $K$ closest tables to the question using the inner product.
Then, during the second-stage ranking stage, a table is chosen among the $K$
using a \emph{semantic relevance model}~\cite{shraga2020web, wang2021retrieving},
that integrates the question and table representation together. 

-----

NL2SQL interfaces \cite {li2014nalir, utama2018end}
translate a natural question into a SQL query that can be evaluated against a
database. In contrast, we concentrate on the data discovery problem: we do not
need to translate natural questions to SQL, instead, we generate SQL from tables
and then text from SQL to automatically generate training data. 

\notera{end - to integrate}

\mypar{Data discovery with sophisticated interafces}
Aurum \cite{fernandez2018aurum} captures and maintain relationships among tables in a collection so that a user can 
find the relevant table more easily. It defines a new domain query language and thus incurs learning cost. 
Auctus \cite{castelo2021auctus} provides, in addtion to keyword query, more diverse interfaces for users to specify spatial, 
temporal and data-integration queries. It also supports multiple constraints fo user to specify. 
Although powerful and flexible, the interface is more application specific  and also requires more skills of the user. 

\mypar{Synthetic question generation from tables and training}
\cite{chemmengath2021topic} automatically generate  questions over a table from the test topic to address 
the topic shift issue in table question answering task, which is different form our task, data discovery.  
They still use the train and test human questions to guide the question generation,  while we only assume the test question is in natural language 
and never use the human questions for question generation. In addtion, they use the synthetic questions as augumntation to real training data, while we use the synthetic questions only and thus face more challenges.

\mypar{Open question answering over tables}
\cite{sun2016table} proposes a very similiar table representation and relevance model as ours to 
select table cells among many tables given a natural language question. They decomose a table into row-wise relation chains  and reduce relevance model to 
relation match. Howerver, there are many differences. First, their table relation chains are mainly for second-stage rank, while we  precompute a semantic vector representation for each relation for first stage retrieval, in addtion, we include the table Title as a important relation node , while they do not.  
Second, for relation match,  they use a Name Entity Recognizer to detect entites (topic entities) in a question and then decompose the question into a question relation chain for each topic entity which is problematic if no entity found. While we treat the question as a whole.  Third, they rely a knowledge base like Freebase to link  the topic entity to table cells to generate table relation chains. They also use the Bing search engine to augment a question to prune the many irelevant table relation chains. While our system only uses released pretrained models. 

\cite{chen2021open} aims to answer a question over a large collection of tables with free context  text around which is mainly for the scenario of documents/web pages containg tables. So both the task and scenario are different because we focus on table collection without much context text except the table caption.  \cite{herzig2021open} also extends OpenDTR to build a question answering system over a table collection to get an answer. 
 
\mypar{Table representation learning}
\cite{deng2020turl} apply an unsupervised pre-traing and supervised finetuning paradigm to learn a table representation. 
They assume there is a topic entity which is extracted from the table caption or the page title for web tables.  
While in data discovery scenario, the table caption may not contain the topic entity and we don't know which column is the topic entity either.
In addition their table represtation is not for large scale search given a natural language question but for scenarios where the input is a table, 
e.g. link a cell of a input table to entities of a knowledage base.  

\cite{herzig2020tapas, eisenschlos2021mate} learn table representations for table question answering 
where a table is always given and then a question is asked for an answer which may be cells in the table or aggreation of cells.
While for data discovery the table has to be retrived by the system itself. 

